On grid homology for lens space links: combinatorial invariance and integral coefficients

Following the approach to grid homology of links in $S^3$, we prove combinatorially that the grid homology of links in lens spaces defined by Baker, Grigsby, and Hedden is a link invariant. Further, using the sign assignment defined by Celoria, we prove that the generalization of grid homology to integral coefficients is a link invariant.

==> macros.tex <==
% Macros

% Typesetting.
\def\co{\colon\thinspace} % Colon for function notation.
\newcommand\lu[1]{\mbox{}^{#1}} % Upper index on the left with better spacing.
\newcommand\li[1]{\mbox{}#1} % Lower/Upper index on the left with better spacing.

% Reference words (to allow customization).
\def\Figure{Figure}
\def\Figures{Figures}
\def\Equation{Eq.}
\def\Equations{Eq.}
\def\Theorem{Theorem}
\def\Theorems{Theorems}
\def\Proposition{Proposition}
\def\Propositions{Propositions}
\def\Lemma{Lemma}
\def\Lemmas{Lemmas}
\def\Section{Section}
\def\Sections{Sections}
\def\Chapter{Chapter}
\def\Chapters{Chapters}
\def\Definition{Definition}
\def\Definitions{Definitions}
\def\Appendix{Appendix}
\def\Appendices{Appendices}
\def\Corollary{Corollary}
\def\Corollaries{Corollaries}
\def\Example{Example}
\def\Examples{Examples}
\def\Conjecture{Conjecture}
\def\Conjectures{Conjectures}

\def\bol{\bf}
\def\example{{\bf {\bigskip}{\noindent}Example: }}
\def\examples{{\bf {\bigskip}{\noindent}Examples: }}
\def\question{{\bf {\bigskip}{\noindent}Question: }}
%\def\remark{{\bf {\bigskip}{\noindent}Remark. }}
\def\note{{\bf {\bigskip}{\noindent}Note: }}
\def\notes{{\bf {\bigskip}{\noindent}Notes: }}
\def\ackn{{\bf {\bigskip}{\noindent}Acknowledgments. }}
\def\bar{\overline}

% Abbreviations.
\newcommand{\pphi}{\varphi}
\newcommand{\s}{_{\ast}}
\newcommand{\bdy}{\partial}
\newcommand{\trr}{\triangleright}
\newcommand{\trl}{\triangleleft}
\newcommand{\sqtens}{\boxtimes} % Square ``bordered'' tensor product.
\newcommand{\ul}{\underline}
\newcommand{\ol}{\overline}
\newcommand{\into}{\hookrightarrow}
\newcommand{\onto}{\twoheadrightarrow}

\newcommand{\ha}{\langle h_A \rangle }
\newcommand{\hd}{\langle h_D \rangle }

\newcommand{\alg}{\mathcal{A}(F)}
\newcommand{\az}{\mathcal{A}(\zz)}
\newcommand{\cala}{\mathcal{A}}
\newcommand{\ainf}{\mathcal{A}_\infty}
\newcommand{\gr}{\textrm{gr}}
\newcommand{\gens}{\mathfrak S}
\newcommand{\hs}{(\mathcal H, \mathfrak s)}
\newcommand{\ghs}{\mathfrak S(\mathcal H, \mathfrak s)}
\newcommand{\grg}{Grothendieck group }
\newcommand{\sss}{{\bf s}}
\newcommand{\ttt}{{\bf t}}
\newcommand{\sso}{{\bf s_0}}
\newcommand{\fs}{f_{\bf s}}
\newcommand{\xx}{{\bf x}}
\newcommand{\yy}{{\bf y}}

% Roman operator/function names.
%\DeclareMathOperator{\obj}{obj}
\DeclareMathOperator{\sut}{sut}
\DeclareMathOperator{\emb}{emb}
\DeclareMathOperator{\Int}{Int}
\DeclareMathOperator{\Inv}{Inv}
\DeclareMathOperator{\inv}{inv}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\spin}{Spin}
\DeclareMathOperator{\rel}{rel}
\DeclareMathOperator{\ev}{ev}
\DeclareMathOperator{\Gr}{Gr}
%\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\op}{op}
\DeclareMathOperator{\PD}{PD}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Mor}{Mor}
\DeclareMathOperator{\Mod}{Mod}
\DeclareMathOperator{\Db}{D}	% Double
\newcommand{\spinc}{\spin^{c}}
\DeclareMathOperator{\BBar}{Bar}
\DeclareMathOperator{\merge}{merge}
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\rank}{rank}

% Caligraphic letters.
\newcommand{\G}{\mathcal{G}}
%\newcommand{\HH}{\mathcal{H}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\zz}{\mathcal Z}
\newcommand{\B}{\mathcal{B}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\TW}{\mathcal{TW}}
\newcommand{\scat}{\mathcal{S}}
\newcommand{\sdcat}{\mathcal{SD}}

% Gothic letters (for Spin-c structures).
%\newcommand{\s}{\mathfrak{s}}
\newcommand{\tsp}{\mathfrak{t}}
\newcommand{\q}{\mathfrak q}

% Blackboard letters.
\newcommand{\A}{\mathbb A}
\newcommand{\C}{\mathbb C}
\newcommand{\Q}{\mathbb Q}
\newcommand{\OO}{\mathbb O}
\newcommand{\XX}{\mathbb X}

% Bold roman letters.
\newcommand{\ZZZ}{\mathbf{Z}}
\newcommand{\aaa}{\mathbf{a}}
\newcommand{\bbb}{\mathbf{b}}
\newcommand{\ccc}{\mathbf{c}}
\newcommand{\ddd}{\mathbf{d}}
\newcommand{\xxx}{\mathbf{x}}
\newcommand{\yyy}{\mathbf{y}}
\newcommand{\zzz}{\mathbf{z}}
\newcommand{\www}{\mathbf{w}}

% Bold symbols.
\newcommand{\bcirc}{\mathbin{\boldsymbol\circ}}
\newcommand{\balpha}{\boldsymbol\alpha}
\newcommand{\bbeta}{\boldsymbol\beta}
\newcommand{\bgamma}{\boldsymbol\gamma}
\newcommand{\btheta}{\boldsymbol\theta}

% Notation.
\newcommand{\cf}{\mathit{CF}}
\newcommand{\ct}{\mathit{CT}}
\newcommand{\hf}{\mathit{HF}}
\newcommand{\cfd}{\mathit{CFD}}
\newcommand{\cfa}{\mathit{CFA}}
\newcommand{\cfaa}{\mathit{CFAA}}
\newcommand{\cfdd}{\mathit{CFDD}}
\newcommand{\cfad}{\mathit{CFAD}}
\newcommand{\cfda}{\mathit{CFDA}}
\newcommand{\cfta}{\mathit{CFAT}}
\newcommand{\cftd}{\mathit{CFTD}}
\newcommand{\cftda}{\mathit{CFDTA}}
\newcommand{\cfk}{\mathit{CFK}}
\newcommand{\cft}{\mathit{CFT}}
\newcommand{\hfk}{\mathit{HFK}}
\newcommand{\kh}{\mathit{Kh}}
\newcommand{\sfh}{\mathit{SFH}}
\newcommand{\cfhat}{\widehat{\cf}}
\newcommand{\hfhat}{\widehat{\hf}}
\newcommand{\cfdhat}{\widehat{\cfd}}
\newcommand{\cfahat}{\widehat{\cfa}}
\newcommand{\cfaahat}{\widehat{\cfaa}}
\newcommand{\cfddhat}{\widehat{\cfdd}}
\newcommand{\cfadhat}{\widehat{\cfad}}
\newcommand{\cfdahat}{\widehat{\cfda}}
\newcommand{\cfkhat}{\widehat{\cfk}}
\newcommand{\hfkhat}{\widehat{\hfk}}
\newcommand{\cftahat}{\widehat{\cfta}}
\newcommand{\cftdhat}{\widehat{\cftd}}
\newcommand{\cfkt}{\widetilde{\cfk}}
\newcommand{\cftt}{\widetilde{\cft}}
\newcommand{\cftdahat}{\widehat{\cftda}}
\newcommand{\cftat}{\widetilde{\cfta}}
\newcommand{\cftdt}{\widetilde{\cftd}}
\newcommand{\cftdat}{\widetilde{\cftda}}
\newcommand{\cfkm}{\cfk^-}
\newcommand{\hfkm}{\hfk^-}
\newcommand{\cfam}{\cfa^-}
\newcommand{\ctm}{\ct^-}
\newcommand{\ctt}{\widetilde{\ct}}

% Misc.
\newcommand{\hha}{\HH^{\alpha}}
\newcommand{\hhb}{\HH^{\beta}}
\newcommand{\hz}{\HH_{\zz}}
\newcommand{\wdd}{\omega_{\DD}}
\newcommand{\dtens}{\mathbin{\widetilde{\otimes}}} % Derived tensor product.
\newcommand{\brho}{\boldsymbol\rho}
\newcommand{\brarrow}{\overrightarrow{\brho}}
\newcommand{\sigbar}{\overline{\Sigma}}
\newcommand{\sigint}{\Int(\Sigma)}
\newcommand{\ebar}{\overline{e}}
\newcommand{\obar}{\overline{o}}
\newcommand{\sbar}{\overline{s}}
\newcommand{\sige}{\Sigma_{\ebar}}
\newcommand{\parrow}{\overrightarrow{P}}
\newcommand{\mt}{\widetilde{\M}}
\newcommand{\mb}{\overline{\M}}
\newcommand{\mbb}{\overline{\overline{\M}}}
\newcommand{\dbar}{\overline{\del}}
\newcommand{\Zbar}{\overline{\Z}}
\newcommand{\Gammabar}{\overline{\Gamma}}
\newcommand{\Pbar}{\overline{P}}
\newcommand{\mubar}{\overline{\mu}}
\newcommand{\mbar}{\overline{m}}
\newcommand{\Grup}{\overline{\Gr}}
\newcommand{\Grdn}{\underline{\Gr}}
\newcommand{\grup}{\overline{\gr}}
\newcommand{\grdn}{\underline{\gr}}


\def\P{\mathcal{P}}
\def\Pp{\boldsymbol{\P}}
\newcommand{\Pdot}[2]{\{\P_.^{#1}\}^{#2}_1}
%\newcommand{\auto}{car}
\def\Ss{\mathcal{S}}
\def\I{\mathcal{I}}
\def\a{\mathbf{a}}
\def\e{\boldsymbol{\epsilon}}
\def\ah{\mathbf{a}_{\frac12}}
\def\b{\mathbf{b}}
\def\bh{\mathbf{b}_{\frac12}}
\def\V{\mathcal{V}}
\def\m{\mathbf{m}}
\def\n{\mathbf{n}}
\def\W{\mathcal{W}}
\def\Inv{\mathrm{Inv}}
\def\stphi{(S,T,\phi)}
\def\H{\mathcal{H}}
\def\E{\mathcal{E}}
\def\Aa{\mathcal{A}}
\def\Cc{\mathcal{C}}
\def\M{\mathcal{M}}
\def\TO{T_\O}
\def\SO{S_\O}
\def\SX{S_\X}
\def\TX{T_\X}
\def\CDA^-{\mathit{CDA}^-}
\def\CATA{\mathit{CATA}}
\def\CDTD{\mathit{CDTD}}
\def\AA{\ensuremath{\mathit{AA}}}
\def\DD{\ensuremath{\mathit{DD}}}
\def\DA{\ensuremath{\mathit{DA}}}
\def\AD{\ensuremath{\mathit{AD}}}

